GoSafe: Globally Optimal Safe Robot Learning

When learning policies for robotic systems from data, safety is a major concern, as violation of safety constraints may cause hardware damage. SafeOpt is an efficient Bayesian optimization (BO) algorithm that can learn policies while guaranteeing safety with high probability. However, its search space is limited to an initially given safe region. We extend this method by exploring outside the initial safe area while still guaranteeing safety with high probability. This is achieved by learning a set of initial conditions from which we can recover safely using a learned backup controller in case of a potential failure. We derive conditions for guaranteed convergence to the global optimum and validate GoSafe in hardware experiments.

==> content/algorithm.tex <==
\tikzset{cross/.style={cross out, draw=blue, very thick, minimum size=0.5em, inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}
\tikzset{cross2/.style={cross out, draw=red, very thick, minimum size=0.5em, inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}
\tikzset{cross3/.style={cross out, draw=green!70!black, very thick, minimum size=0.5em, inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}
\subfloat[\label{sfig:stage1}]{%
\begin{tikzpicture}
\node[draw, rectangle, minimum width=9.5em, minimum height=8em, pattern=north west lines, pattern color=darkgray, opacity=0.9](plot){};
% \node[draw, regular polygon, regular polygon sides=6, rounded corners, minimum size=5em, above=0em of plot.south, inner sep=0, fill=white](safe1){};
\node at($(plot.south)+(0.5em, 2em)$)(safe1) {\tikz\asymcloud[.075]{fill=white};}; 
\node[draw=none, ellipse, minimum width=3em, minimum height=1.5em, below right = 2em and 1em of plot.north west, fill=white](safe2){};
% \node[draw, ellipse, minimum width=1.5em, minimum height=3em, below left = 2em and 1em of plot.north east](safe3){};
% \node[draw, ellipse, minimum width=1em, minimum height=3em, below right = 4em and 2em of plot.north west](safe4){};
% \node[draw, rectangle, minimum width=0.75em, minimum height=1.8em, above left=0.5em and 2em of safe1.north east, anchor=south east, fill=white](safe4){};
\node[draw=none, ellipse, minimum width=3em, minimum height=0.5em, below right = 3.5em and 0.25em of plot.north, fill=white, rotate=-30](safe5){};
\node[draw=none, ellipse, minimum width=1em, minimum height=2em, below = 0.5em of plot.north, fill=white](safe6){};
%
\draw[dashed] (plot.south)node[below]{$x_0$} -- (plot.north);
\draw[dashed] ($(plot.west)+(0em, -3em)$)node[left]{$a_0$} -- ($(plot.east)+(0em, -3em)$);
\draw[green!70!black, line width=3pt]($(plot.south)+(0em,0.25em)$) -- ($(plot.south)+(0em,2.75em)$);
%
\node[draw, cross, above=2em of plot.south](opt){};
\node[above left=3em and 1em of plot.west, rotate=90]{Parameter $a$};
%
\node[draw, rectangle, fill=white, below left=0.5em and 0.5em of plot.north east]{\ref{item:S1}};
\end{tikzpicture}
}
%%%%%
%%%%%
\subfloat[\label{sfig:stage2}]{%
\begin{tikzpicture}
\node[draw, rectangle, minimum width=9.5em, minimum height=8em, pattern=north west lines, pattern color=darkgray, opacity=0.9](plot){};
\node at($(plot.south)+(0.5em, 2em)$)(safe1) {\tikz\asymcloud[.075]{fill=green!70!black};}; 
\node[draw=none, ellipse, minimum width=3em, minimum height=1.5em, below right = 2em and 1em of plot.north west, fill=white](safe2){};
% \node[draw, ellipse, minimum width=1.5em, minimum height=3em, below left = 2em and 1em of plot.north east](safe3){};
% \node[draw, ellipse, minimum width=1em, minimum height=3em, below right = 4em and 2em of plot.north west](safe4){};
% \node[draw, rectangle, minimum width=0.75em, minimum height=1.8em, above left=0.5em and 2em of safe1.north east, anchor=south east, fill=white](safe4){};
\node[draw=none, ellipse, minimum width=3em, minimum height=0.5em, below right = 3.5em and 0.25em of plot.north, fill=green!70!black, rotate=-30](safe5){};
\node[draw=none, ellipse, minimum width=1em, minimum height=2em, below = 0.5em of plot.north, fill=white](safe6){};
%
\draw[dashed] (plot.south)node[below]{$x_0$} -- (plot.north);
\draw[dashed] ($(plot.west)+(0em, -3em)$)node[left]{$a_0$} -- ($(plot.east)+(0em, -3em)$);
%
\node[draw, cross, above=4em of plot.south](opt){};
%
\node[draw, rectangle, fill=white, below left=0.5em and 0.5em of plot.north east]{\ref{item:S2}};
\end{tikzpicture}
}
%%%%%

%%%%%
\subfloat[\label{sfig:stage3}]{%
\begin{tikzpicture}
\node[draw, rectangle, minimum width=9.5em, minimum height=8em, pattern=north west lines, pattern color=darkgray, opacity=0.9](plot){};
\node at($(plot.south)+(0.5em, 2em)$)(safe1) {\tikz\asymcloud[.075]{fill=green!70!black};}; 
\node[draw=none, ellipse, minimum width=3em, minimum height=1.5em, below right = 2em and 1em of plot.north west, fill=white](safe2){};
% \node[draw, ellipse, minimum width=1.5em, minimum height=3em, below left = 2em and 1em of plot.north east](safe3){};
% \node[draw, ellipse, minimum width=1em, minimum height=3em, below right = 4em and 2em of plot.north west](safe4){};
% \node[draw, rectangle, minimum width=0.75em, minimum height=1.8em, above left=0.5em and 2em of safe1.north east, anchor=south east, fill=white](safe4){};
\node[draw=none, ellipse, minimum width=3em, minimum height=0.5em, below right = 3.5em and 0.25em of plot.north, fill=green!70!black, rotate=-30](safe5){};
\node[draw=none, ellipse, minimum width=1em, minimum height=2em, below = 0.5em of plot.north, fill=white](safe6){};
%
\draw[dashed] (plot.south)node[below]{$x_0$} -- (plot.north);
\draw[dashed] ($(plot.west)+(0em, -3em)$)node[left]{$a_0$} -- ($(plot.east)+(0em, -3em)$);
%
% \node[draw, cross2, left=0.5em of safe1](opt){};
\node[draw, cross2, below left=0em and 1em of safe5](opt){};
% \node[draw, cross2, right=0.5em of safe1](opt){};
% \node[draw, cross2, above right=0.5em and 1em of safe5](opt){};
\node[draw, cross2, below left = 1em and 1.5em of safe5]{};
\node[draw, cross2, above right = 0.5em and 0.5em of safe1.north]{};
\node[draw, cross, above=4em of plot.south](opt){};
\node[draw, cross3, right=2.5em of safe2.west](curr){};
\node[above left=3em and 1em of plot.west, rotate=90]{Parameter $a$};
\node[below=1em of plot, inner sep=0]{Initial condition $\tilde{x}_0$};
%
\node[draw, rectangle, fill=white, below left=0.5em and 0.5em of plot.north east]{\ref{item:S3}};
\end{tikzpicture}
}
%%%%%
%%%%%
\subfloat[\label{sfig:stage4}]{%
\begin{tikzpicture}
\node[draw, rectangle, minimum width=9.5em, minimum height=8em, pattern=north west lines, pattern color=darkgray, opacity=0.9](plot){};
\node at($(plot.south)+(0.5em, 2em)$)(safe1) {\tikz\asymcloud[.075]{fill=green!70!black};}; 
\node[draw=none, ellipse, minimum width=3em, minimum height=1.5em, below right = 2em and 1em of plot.north west, fill=green!70!black](safe2){};
% \node[draw, ellipse, minimum width=1.5em, minimum height=3em, below left = 2em and 1em of plot.north east](safe3){};
% \node[draw, ellipse, minimum width=1em, minimum height=3em, below right = 4em and 2em of plot.north west](safe4){};
% \node[draw, rectangle, minimum width=0.75em, minimum height=1.8em, above left=0.5em and 2em of safe1.north east, anchor=south east, fill=white](safe4){};
\node[draw=none, ellipse, minimum width=3em, minimum height=0.5em, below right = 3.5em and 0.25em of plot.north, fill=green!70!black, rotate=-30](safe5){};
\node[draw=none, ellipse, minimum width=1em, minimum height=2em, below = 0.5em of plot.north, fill=green!70!black](safe6){};
%
\draw[dashed] (plot.south)node[below]{$x_0$} -- (plot.north);
\draw[dashed] ($(plot.west)+(0em, -3em)$)node[left]{$a_0$} -- ($(plot.east)+(0em, -3em)$);
% \draw[very thick, green!70!black] (safe6.south) -- (safe6.north);
%
\node[draw, cross2, left=0.5em of safe1](opt){};
\node[draw, cross2, below left=0em and 1em of safe5](opt){};
% \node[draw, cross2, right=0.5em of safe1](opt){};
% \node[draw, cross2, above right=0.5em and 1em of safe5](opt){};
\node[draw, cross2, above=5em of plot.south]{};
\node[draw, cross2, below left = 1em and 1.5em of safe5]{};
\node[draw, cross2, above right = 0.5em and 0.5em of safe1.north]{};
\node[draw, cross, above=6em of plot.south](opt){};
\node[below=1em of plot, inner sep=0]{Initial condition $\tilde{x}_0$};
%
\node[draw, rectangle, fill=white, below left=0.5em and 0.5em of plot.north east]{End};
\end{tikzpicture}
}
%%%%%

% %%%%%
% \subfloat[\label{sfig:exp_success}]{%
% \begin{tikzpicture}
% \node[draw, rectangle, minimum width=7.5em, minimum height=8em](plot){};
% \draw[dashed]($(plot.west)+(0em,3em)$)node[left]{$g_1$} -- ($(plot.east)+(0em,3em)$);
% \draw[dashed]($(plot.west)+(0em,2em)$)node[left]{$\partial{S}_n$} --node[pos=0.4](halfway){} ($(plot.east)+(0em,2em)$);
% %
% \node[coordinate, above=2em of plot.south west](start){};
% \node[coordinate, below=1em of halfway](middle){};
% \node[coordinate, above=4em of plot.south east](end){};
% \draw (start)node[left]{$x_0$} to[out=70, in=180] (middle);
% \draw (middle) to[out=0, in=-110] (end)node[right](xdes){$x_\mathrm{des}$};
% %
% \node[above left=3em and 2em of plot.west, rotate=90]{State $x(t)$};
% \node[below=1em of plot]{Time $t$};
% \draw (plot.south west)node[below]{0} -- (plot.north west);
% \draw (plot.south east)node[below]{$t_\mathrm{e}$} -- (plot.north east);
% %
% \node[draw, rectangle, inner sep=0, minimum width=0.5em, fill=black] at(xdes-|plot.east){};
% \node[draw, rectangle, inner sep=0, minimum width=0.5em, fill=black] at(start){};
% \end{tikzpicture}
% }
% %%%%%
% %%%%%
% \subfloat[\label{sfig:exp_fail}]{%
% \begin{tikzpicture}
% \node[draw, rectangle, minimum width=7.5em, minimum height=8em](plot){};
% \draw[dashed]($(plot.west)+(0em,3em)$)node[left]{$g_1$} -- ($(plot.east)+(0em,3em)$);
% \draw[dashed]($(plot.west)+(0em,2em)$)node[left]{$\partial{S}_n$} --node[cross2,solid,pos=0.4](halfway){} ($(plot.east)+(0em,2em)$);
% %
% \node[coordinate, above=4em of plot.south west](start){};
% \node[coordinate, below=0em of halfway](middle){};
% \node[coordinate, above=2em of plot.south east](end){};
% \node[coordinate, above=4em of plot.south east](end_opt){};
% \draw (start)node[left]{$\tilde{x}_0$} to[out=20, in=220] (halfway);
% \draw (halfway) to[out=-20, in=-110] (end);
% %
% % \node[above left=2.5em and 2em of plot.west, rotate=90]{State $x(t)$};
% \node[below=1em of plot, inner sep=0]{Time $t$};
% \draw (plot.south west)node[below]{0} -- (plot.north west);
% \draw (plot.south east)node[below]{$t_\mathrm{e}$} -- (plot.north east);
% \draw (plot.south east) -- (end_opt)node[right](xdes){$x_\mathrm{des}$};
% \draw[<-] (halfway) -- +(0.75em, -3em)node[below,align=center]{switch to\\backup controller};
% %
% \node[draw, rectangle, inner sep=0, minimum width=0.5em, fill=black] at(xdes-|plot.east){};
% \node[draw, rectangle, inner sep=0, minimum width=0.5em, fill=black] at(start){};
% \end{tikzpicture}
% }
